Analytical Calculation of Four-Point Correlations for a Simple Model of Cages Involving Numerous Particles

Dynamics of a one-dimensional system of Brownian particles with short-range repulsive interaction (diameter sigma) is studied with a liquid-theoretical approach. The mean square displacement, the two-particle displacement correlation, and the overlap-density-based generalized susceptibility are calculated analytically by way of the Lagrangian correlation of the interparticulate space, instead of the Eulerian correlation of density that is commonly used in the standard mode-coupling theory. In regard to the mean square displacement, the linear analysis reproduces the established result on the asymptotic subdiffusive behavior of the system. A finite-time correction is given by incorporating the effect of entropic nonlinearity with a Lagrangian version of mode-coupling theory. The notorious difficulty in derivation of the mode-coupling theory concerning violation of the fluctuation-dissipation theorem is found to disappear by virtue of the Lagrangian description. The Lagrangian description also facilitates analytical calculation of four-point correlations in the space-time, such as the two-particle displacement correlation. The two-particle displacement correlation, which is asymptotically self-similar in the space-time, illustrates how the cage effect confines each particle within a short radius on one hand and creates collective motion of numerous particles on the other hand. As the time elapses, the correlation length grows unlimitedly, and the generalized susceptibility based on the overlap density converges to a finite value which is an increasing function of the density. The distribution function behind these dynamical four-point correlations and its extension to three-dimensional cases, respecting the tensorial character of the two-particle displacement correlation, are also discussed.

==> kanjicollab.tex <==
% ------------------------------------------------------------------------
\author{\surname{Ooshida} Takeshi (Âç¿®ÅÄ ¾æ»Ö)}
\email[E-mail:~]{ooshida@damp.tottori-u.ac.jp}
\affiliation{%
   Department of Mechanical and Aerospace Engineering,
   % Graduate School of Engineering, 
   Tottori University, Tottori 680-8552, Japan}
% ------------------------------------------------------------------------
\author{Susumu \surname{Goto} (¸åÆ£ ¿¸)}
\affiliation{%
   Graduate School of Engineering Science,  
   Osaka University, 
   \relax{Toyonaka, Osaka 560-8531, Japan}}
% ------------------------------------------------------------------------
\author{Takeshi \surname{Matsumoto} (¾¾ËÜ ¹ä)}
\affiliation{%
   Division of Physics and Astronomy, Graduate School of Science, 
   Kyoto University, 
   \relax{Kyoto 606-8502, Japan}}
% ------------------------------------------------------------------------
\author{Akio \surname{Nakahara} (Ã渶 ÌÀÀ¸)}
\affiliation{%
   Laboratory of Physics, College of Science and Technology,
   Nihon University, 
   \relax{Funabashi, Chiba 274-8501, Japan}}
% ------------------------------------------------------------------------
\author{Michio \surname{Otsuki} (ÂçÄÐ Æ»É×)}
\thanks{%
   Present address:
   Department of Materials Science, 
   Shimane University, 
   Matsue 690-8504, Japan}
\affiliation{%
   Department of Physics and Mathematics, Aoyama Gakuin University, 
   % Fuchinobe-5-10-1, 
   \relax{Sagamihara, Kanagawa 229-8558, Japan}}
% ------------------------------------------------------------------------


